The Unreasonable Effectiveness of Address Clustering

Address clustering tries to construct the one-to-many mapping from entities to addresses in the Bitcoin system. Simple heuristics based on the micro-structure of transactions have proved very effective in practice. In this paper we describe the primary reasons behind this effectiveness: address reuse, avoidable merging, super-clusters with high centrality, and the incremental growth of address clusters. We quantify their impact during Bitcoin's first seven years of existence.

==> Makefile <==
TEXFILES = main.tex tex/conc.tex tex/formation.tex tex/related.tex \
           tex/abstract.tex tex/counts.tex tex/intro.tex tex/sizes.tex
IMGFILES = img/co-spents/co-spents.png img/counts/counts.png \
           img/increases/increases.png img/ratios/ratios.png \
           img/ratios/ratios-annotated.png img/sizes/sizes.png \
           img/top-address-clusters/top-address-clusters.png
BIBFILES = bib/main.bib

.PHONY: all clean

all: main.pdf

main.pdf: $(TEXFILES) $(IMGFILES) $(BIBFILES)
	latexmk -pdf -use-make $<

clean:
	latexmk -CA

